Dataflow-Architecture Co-Design for 2.5D DNN Accelerators using Wireless Network-on-Package

Deep neural network (DNN) models continue to grow in size and complexity, demanding higher computational power to enable real-time inference. To efficiently deliver such computational demands, hardware accelerators are being developed and deployed across scales. This naturally requires an efficient scale-out mechanism for increasing compute density as required by the application. 2.5D integration over interposer has emerged as a promising solution, but as we show in this work, the limited interposer bandwidth and multiple hops in the Network-on-Package (NoP) can diminish the benefits of the approach. To cope with this challenge, we propose WIENNA, a wireless NoP-based 2.5D DNN accelerator. In WIENNA, the wireless NoP connects an array of DNN accelerator chiplets to the global buffer chiplet, providing high-bandwidth multicasting capabilities. Here, we also identify the dataflow style that most efficienty exploits the wireless NoP's high-bandwidth multicasting capability on each layer. With modest area and power overheads, WIENNA achieves 2.2X--5.1X higher throughput and 38.2% lower energy than an interposer-based NoP design.

==> Tables/DataflowTable.tex <==
\begin{table*}[t]
\centering
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{0pt}
\scriptsize
  
\begin{tabular} {|@{~} l @{~}|p{3cm}|p{3cm}|p{3cm}|p{2cm}|}
\hline
\multicolumn{1}{|@{~} c @{~}|}{\textbf{Strategy Name}} 
& \multicolumn{1}{@{~} c @{~}|}{\textbf{Partitioned dim. across Chiplets}} 
& \multicolumn{1}{@{~} c @{~}|}{\textbf{Partitioned dim. within Chiplets}} 
& \multicolumn{1}{@{~} c @{~}|}{\textbf{Broadcasted tensor}} 
& \multicolumn{1}{@{~} c @{~}|}{\textbf{Unicasted tensor}}  \\
\hline

Filter-channel partitioned (KP-CP)
& Filter (K)
& Channel (C)
& Input Activation
& Filter Weight  \\
\hline

Batch-channel partitioned (NP-CP)
& Activation Batch (N)
& Channel (C)
& Filter Weight
& Input Activation  \\
\hline

Row-column partitioned (YP-XP)
& Output activation row (Y')
& Output activation column (X')
& Input Activation
& Filter Weight  \\
\hline


 \end{tabular}
  \caption{\small Dataflow styles we charaterize and their characteristics. In spatial reuse column, "M" and "B" indicate multicast and broadcast, respectively. In loop order column, red texts represent parallelized dimension, and "/" indicates another PE hierarchy level. In tile size column, absolute symbol on a dimension  (e.g., $|X|$) represent the size of the corresponding dimension in a layer. 
  %Some parameters such as the cluster size of NVDLA dataflow are co-optimized with hardware design parameters, thus they follow hardware design parameters. We mark such parameters using "P" followed by their names. Also, some mapping sizes such as the mapping size of K in Eyeriss dataflow is not specified thus free-variables. We select such free-variables to be minimum in this work.
  \vspace{-5mm} }
  \label{table:dataflows}
\end{table*}



==> backup/00-abstract.tex <==
Deep neural networks (DNNs) have emerged as enablers of many classification and segmentation tasks with super-human accuracy. To efficiently provide low-latency inference of large DNNs, hardware accelerators are being developed and deployed on edge devices and in datacenters.
However, complex DNN models continue to become larger and more complex, they demand increasing compute to meet the target latency and throughput characteristics for real-time inference.
This naturally requires an efficient scale-out mechanism for increasing compute density.
2.5D integration over interposer has emerged as a promising solution, but as we show in this work, the limited bandwidth offered by the interposer and multiple hops in mesh topology can diminish the benefits of scaled out accelerators. % the number of chiplets.
%Deep neural networks (DNNs) have emerged as enablers of many classification and segmentation tasks with super-human accuracy. To efficiently support the processing of large DNNs, hardware DNN accelerators have been developed. Although DNN accelerator chips provide orders of magnitude improvements in throughput and energy efficiency, they are designed for a particular network size and lack flexibility to adapt to different problems. Moreover, scaling up such monolithic chips to cater the increasing needs of large DNNs introduces important manufacturing cost challenges. Alternatively, interposer-based 2.5D designs have emerged as a promising solution to these issues. In this case, the architecture can be scaled out by integrating multiple accelerator chiplets within the same package and communicating them through the interposer. However, the limited bandwidth offered by the interposer can become a performance bottleneck, diminishing the benefits of increasing the number of chiplets.
To cope with the inter-chiplet bandwidth challenge, we propose \ourwork, a wireless network-on-package-based 2.5D DNN accelerator.
%\ourwork consists of a SRAM-based global buffer chiplet backed by high-bandwidth memory (HBM) and a DNN accelerator chiplet array.
In \ourwork, a wireless Network-on-Package (NoP) connects an array of DNN accelerator chiplets to the global buffer chiplet, providing high-bandwidth multicasting capabilities.
\ourwork also identifies the most efficient dataflow style among three distinct styles tuned for wireless NoP's high-bandwidth multicasting capability on each layer.
%required by DNN workloads.
\ourwork shows substantial improvements in terms of latency and energy efficiency with respect to an interposer-network-based design, while incurring low area overhead.
%\TODO{sprinkle the word co-design in abstract and intro}

% Deep neural network (DNN) has emerged as an enabler of many classification and segmentation tasks with super-human accuracy.
% To efficiently support DNNs that includes billions of computation with millions of parameters, hardware specialized for DNNs called a DNN accelerator has been developed.
% Although DNN accelerator chips provided orders of magnitude improvements in throughput and energy efficiency, systems deploying DNN accelerator chips started require exponential increase of the number of compute units within each DNN accelerator chip to sustain recent DNN workloads with a larger number of DNN models.
% However, since larger chips introduce manufacturing cost challenges, scaling up a monolithic design is not a promising solution.
% Alternatively, interposer-based 2.5D designs, which employs multiple chiplets within a package, emerged as one of the most promising solutions.
% Interposer-based 2.5D designs facilitated scaling up a DNN accelerator chip. However, the limited bandwidth of interconnection network among chiplets started bottleneck the performance of the entire chip, diminishing the benefits of the larger number of compute units. 

% To cope with the inter-chiplet bandwidth challenge, we propose \ourwork, a wireless network-on-package-based 2.5D DNN accelerator chip.
% \ourwork consists of SRAM-based global buffer chiplet backed by high-bandwidth memory (HBM) and a DNN accelerator chiplet array.
% A wireless network interconnects each DNN accelerator chiplet and the global buffer chiplet, providing high-bandwidth multicasting capabilities required by DNN workloads.
% In our evaluation, \ourwork provided XX\% lower latency and YY\% higher energy efficiency on average compared to a baseline interposer network-based design with only ZZ\% of area overhead.


%\ac{CNN}, one of the most relevant AI algorithms, achieve outstanding results at several different applications by computing billions of operations between their parameters. This comes at a computational and communication cost at the processors level, which has forced the hardware evolve from CPUs and GPUs to specific accelerators for neural networks. These accelerators currently rely on traditional Networks-on-Chip (NoC) to interconnect the cores within a die, but the exponential growth on the number of cores in the designs is making the whole system to require more flexible and scalable NoCs to avoid becoming a bottleneck. In order to overcome this same situation in general manycore systems, \ac{WNoC} have been proposed and proved effective. 
%This paper proposes an scalable solution for CNN accelerators by using WNoCs, which as opposed to electrical NoCs provide demanded properties like broadcasting and low latency support, while taking into account crucial requirements for neural network inference such as dataflows adaptability.

%Convolutional Neural Networks (CNN), one of the most relevant AI algorithms, achieve outstanding results at several different applications by computing billions of operations between their parameters. This comes at a computational and communication cost at the processors level, which has forced the hardware evolve from CPUs and GPUs to specific accelerators for neural networks. These accelerators currently rely on traditional Networks-on-Chip (NoC) to interconnect the cores within a die, but the exponential growth on the number of cores in the designs is making the whole system to require more flexible and scalable NoCs to avoid becoming a bottleneck. In order to overcome this same situation in general manycore systems, Wireless Network-on-Chip (WNoC) have been proposed and proved effective. 
%This paper proposes an scalable solution for CNN accelerators by using WNoCs, which as opposed to electrical NoCs provide demanded properties like broadcasting and low latency support, while taking into account crucial requirements for neural network inference such as dataflows adaptability.



==> backup/01-introduction.tex <==
\section{Introduction}
\label{sec:intro}
%\vspace{-2mm}

% 1 frase de cada paragraf.
%1.	ML exploded…. coses guays de AI
%2.	processing al integrar ML. efficiency importancia…
%3.	Acceleradors. Busquem minim consum amb maxima performance. Son bastant adequats per ML.
%4.	importancia communciations, normalment obviades. Referencia a alguns papers que tinguin en compte les comunicacions
%5.	Problema comunicacions: encara challenge, efficiency, flexible..
%6.	Wireless com a alternativa nova. Ventatges(broad/latency/distance indp). Acronym.
%7.	Performance numbers, simulation numbers… The remainder of the paper is structure as follows: section II …..



%\textcolor{red}{ML/AI}: 
Recent advancements in the field of Machine Learning (ML) demonstrate that the 
ability of Deep Neural Networks (DNN) to solve tasks such as image classification~\cite{krizhevsky2012imagenet} or pose estimation~\cite{vision} is improving at an unprecedented rate.
%Specifically, Convolutional Neural Networks (CNN) are well suited to object recognition and identification problems.
%Astonishing results such as CycleGAN \cite{Zhu2017UnpairedIT} are a clear sign that both the research community and the industry are really driving this Artificial Intelligence (AI) revolution, which some say will lead the humanity to a new era.
%
%\textcolor{red}{processing needs, accelerators}:
To achieve these outstanding results and accuracy, DNN designs have become larger and deeper, reaching billions of parameters in some cases.
%and being called Deep Neural Networks (DNN) as a consequence.
%These represent huge computational loads for the processors, which not only need to perform well when computing, but also need to take into account the demanding communication requirements. These requirements increase together, but not necessarily linearly, with the computational costs.
Due to the enormous amount of calculations, the hardware running DNN inference has to be energy efficient to ensure the maximum performance at a reduced cost, a goal that CPUs and even GPUs do not live up to easily.
This has led to a fast development of DNN accelerators, specialized hardware architectures designed to match the demands of those algorithms. 


Research in novel DNN accelerators \cite{eyeriss2,maeri} is a bustling topic since data reuse and parallelism opportunities provided by DNNs can be accelerated via custom memory hierarchies and a sea of processing elements (PEs), respectively. However, as DNN models continue to scale, demands to scale the compute capabilities of DNN accelerators is increasing.
%there is a corresponding need to scale the compute capabilities of DNN accelerators.
%\TODO{RG: cite Eyeriss V2? }

At a fundamental level, DNN accelerators can either be scaled via scale-up (i.e., adding more PEs to the accelerator), or scale-out (i.e., connecting multiple accelerator chips together).
There is a natural limit 
to scale-up due to cost and yield issues. 
Scale-out is typically done 
via board-level integration
which comes with overheads of high communication
latency and low bandwidth.
However, the recent appeal of 2.5D integration of multiple ``chiplets" interconnected 
via an interposer on the same package~\cite{chips_dac2019} (e.g., AMD's Ryzen CPU), offers opportunities for enabling efficient scale-out.
The 2.5D integration technology is also proven effective in DNN accelerator domain via recent works~\cite{zimmer20190, shao2019simba}.

%recent appeal of 
%2.5D integration~\cite{Kim2019ArchitectureCA}
%offers opportunities for %enabling efficient scale-out.
%- with multiple 
%research efforts under-way to 
%enable multiple ``chiplets" 
%on the same package, %interconnected 
%via an interposer.

Unfortunately, as we identify in this work, DNN accelerator chiplets have an insatiable appetite for data to keep the PEs utilized, which is a challenge for interposer due to limited bandwidth.
The bandwidth limitations originate from large microbumps ($\sim$40$\upmu$m~\cite{chips_dac2019}) at I/O ports of each chiplet, which naturally reduces the bandwidth by orders of magnitude compared to the nm pitch wires within 
each accelerator chiplet.
Also, since chiplets are often connected via neighbor-to-neighbor connections due to limited I/O bandwidth of chiplets, the number of intermediate chiplets (number of hops) to pass for a data packet to reach its destination increases as the number of chiplets scales.
This also introduces significant amount of delay for data communication latency.

%\TODO{@Hyoukjun - also mention the hop by hop latency limitations}

%DNN computational needs
%the perfect fit between the accelerators and the neural network computational needs. These specific hardware designs can easily leverage the peculiarities of NN algorithms, such as data reuse and parallelism opportunities, which will be discussed later. Due to this reason, accelerators manage ML inference way more pleasantly and efficiently than non-specific architectures.

%\HK{I think we also need to motivate multi-chip DNN accelerators since we target it.} \RG{Added some sentences.}

%\textcolor{red}{flex. scalab. challenges}:

To address these challenges,
we explore opportunities provided by mm-wave wireless 
to serve the data distribution needs of a 2.5D DNN accelerator.
In particular, we identify that
wireless links can (i) provide 
higher bandwidth than their 
electrical interposer counterpart, 
and, more importantly (ii) naturally 
support broadcasts, 
making them a natural fit to 
leverage input and/or weight reuse opportunities
across accelerator chiplets.
To exploit such properties, we also explore dataflow styles optimized to utilize high bandwidth and broadcast capability. 
%\TODO{@Hyoukjun - add a line here on the fact that this paper demonstrates dataflow-microarch-technology co-design: dataflow that leverages spatial reuse via broadcasts, and use on-package wireless which is broadcast friendly}

We present WIENNA, \emph{WIreless-Enabled communications in Neural Network Accelerator}, a
2.5D on-package scale-out accelerator architecture that leverages 
single-cycle
wireless broadcasts to distribute weights and inputs,
depending on the partitioning (i.e., dataflow)
strategy.
We implement three partitioning strategies - batch, filter and activation for the 
scale-out architecture - leveraging the parallelism in DNNs across these three dimensions.
We evaluate an instance of WIENNA targeting 32 TOPS 
by interconnecting 256 
NVDLA~\cite{nvdla}-like accelerator chiplets, and observe 
2.5-4.4$\times$ throughput improvement over a baseline 2.5D accelerator that uses an electrical-only interposer.

%\SA{what about something like: scaled-out WIreless-Enabled Neural Network Accelerators (WIENNA)?}, that 
%interconnects 
%WIENNA leverages 
%wireless broadcasts to distribute weights, inputs and (weights+overapped inputs), respectively, in the three 
%partitioning schemes, 
%thereby increasing the effective bandwidth of the interposer.
%WIENNA provides \TODO{TODO} 

%However, DNN accelerators still face key challenges, especially in terms of communication. 
%One one hand, different DNN 
%layers exhibit different 
%parallelism opportunities, which can be leveraged via 
%appropriate data mappings, known as \textit{dataflows}.
%Within the accelerator, 
%this translates to diverse 
%communication requirements, demanding flexibility from the 
%communication fabric. On the other hand, accelerators must scale up in order to handle massive sizes of data, a non-trivial task if we do not want to compromise the efficiency.
%While these communication requirements are of an utmost importance in the accelerator design and can have a tremendous impact on throughput and latency, very few papers have taken them into account as first-order metrics \cite{maeri}. 
%%and they are often set aside for the enhancement of the computational performance.
%%Even though the computational requirements must be met, it has been proven that the data movement is much more expensive~\cite{eyeriss} in consumption terms.
%\textcolor{red}{NoCs problems}:



%Nonetheless, current accelerators rely on traditional \ac{NoC} to provide the communication links between cores in the same die. While this technology has been very suitable in systems where the number of cores is not massive, modern frameworks are embodying larger amounts of processors, in part due to the exponential miniaturization of the components throughout the years. Moreover, multi-chip neural network accelerators are the state-of-the-art enablers of scalable DNN hardware. Monolithic devices are not well suited to tackle diverse network sizes and purposes within the same system, but interconnecting multiple chips in a die is not trivial. In this scenario, the NoCs performance is lagging behind and it is starting to become a bottleneck.


%To overcome the limitations of NoCs in manycore systems, the community has introduced the Wireless Network-on-Chip (WNoC) paradigm, an alternative to wired topologies that provides flexibility, scalability and many other advantages such as native broadcast support and latency reduction. In this sense, WNoC seem like a suitable technology to be used in DNN accelerators, being the aim of this work exploring such fit.
%In this paper, the WNoC approach will be applied to DNN accelerators, a manycore-like environment that can widely benefit from it. Leveraging a preliminary analysis, we propose WIreless-Enabled communications in Neural Network Accelerator (WIENNA), a DNN accelerator architecture that allows taking advantage of the WNoC technology and improves by XXXXXXX the baseline accelerators. 


%\TK{Can remove the following para to save space}
%The remainder of this paper is organized as follows. Section II provides relevant background in DNN accelerators and the dataflow traffic inside them, as well as context for wireless in-package communications. Section III motivates this work by exploring the inter-chiplet bandwidth impact on overall performance. Section IV presents the WIENNA architecture and Section V evaluates it. Section VI discusses related work and Section VII concludes.




%Section IV introduces the transceivers models and the tools used.





==> backup/02-background.tex <==
\section{Background}
\label{sec:background}

%DNN accelerators in general. (PEs, hw, mac units, noc, point to point comms, tree (what people have done)), including dataflows (diferent reuses opportunities, different broadcast patterns, but difficulties with broadcasts...). Interposer networks packaging..

\insertFigure{Conv2D}{Convolution operation \vspace{-2mm}}
%\subsection{CNN Operations}
%\label{sec:deepneuralnetworks}



%The convolution operation accounts for more than 90\% of total computation in many CNNs~\cite{eyeriss}.
%
%As illustrated in~\autoref{fig:Conv2D}, % convolution is similar to stencil operations that slide a kernel (i.e., sliding window) over an input, computing element-wise multiplication and accumulation of all the multiplication results within each sliding window.
%convolution involves three high-dimensional tensors: 3D input activation, 4D filter weight, and 3D output activation.
%
%When we consider batches, all the tensors become 4D tensors.
%

\begin{figure*}[!t]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-4pt}
\centering
\vspace{-0.1cm}
\includegraphics[width=0.47\textwidth]{./fig/dr_area2}
\hspace{0.3cm}t
%\includegraphics[width=0.47\textwidth]{./fig/dr_power_BER5}
\includegraphics[width=0.45\textwidth]{./fig/dr_power_BER9} % This is for BER9
%\includegraphics[width=0.45\textwidth]{./fig/dr_power_BER12} % This is for BER12
\caption{Area and power for the transceivers as functions of the offered datarate in \cite{Tasolamprou2019, Yu2014, Tokgoz2018} and references therein. Power is normalized for error rate (to 10\textsuperscript{-9}) and transmission range. Energy per bit can be obtained dividing the power by the datarate. 
%\TODO{put these next to each other in one row to get space.}
}
\label{fig:area_dr}\label{fig:power_dr}
\vspace{-0.2cm}
\end{figure*} 

% \begin{figure}[!t]
% \setlength{\abovecaptionskip}{0pt}
% \setlength{\belowcaptionskip}{-4pt}
% \centering

% %\vspace{-0.2cm}
% \caption{\it Wireless transceivers power \cite{Tasolamprou2019, Yu2014, Thyagarajan2015, Tokgoz2016, Dolatsha2017, Tokgoz2018} and references therein}
% \label{fig:power_dr}
% %\vspace{-0.4cm}
% \end{figure} 

\subsection{DNN accelerators}
\label{sec:dnnaccelerators}

A DNN accelerator is specialized hardware for running DNN algorithms, which provides higher throughput and energy-efficiency than GPUs and CPUs via parallelism and dedicated circuitry.
%
The abstract architecture of most DNN accelerators~\cite{eyeriss, flexflow, maeri} consists of an off-chip memory, a global shared memory, and an array of processing elements (PEs) connected via a Network-on-Chip (NoC). 
%Since in a CNN the most often computed operation (around 90\% of total computation) and the most expensive one is the convolution~\cite{eyeriss}, illustrated in~\autoref{fig:Conv2D}, DNN accelerators are mainly focused on optimizing Multiply and Accumulate (MAC) operations. %between an input activation and a filter in each PE.
%The abstract architecture of a DNN accelerator system consists of an off-chip memory, a global shared memory (L3 scratchpad memory), and multiple computing tiles interconnected via various network-on-chip (NoC). %chiplets accessing to it.
%Each computing tile consists of a local shared memory (L2 scratchpad memory), a PE array, and NoC to interconnect them all.
%

%Each of those chiplets are in themselves smaller accelerators, consisting of an array of \ac{PE}, a shared memory and a \ac{NoC} to interconnect the cores and the memory.
%The PEs are made of one or more MAC units and can contain small buffers.


%Each PE contains one or more MAC units and a local private scratchpad memory (L1 scratchpad memory).
%
%To scale out the design, multi-chip package-based DNN accelerators are emerging~\cite{zimmer20190}.
%

%\textcolor{red}{dataflows: }

\betterparagraph{Dataflow} When mapping the targeted neural network into the PEs, several different strategies, or \textit{dataflows}, can be applied. This dataflow space is huge and its exploration is an active research topic~\cite{maestro, gao2019tangram, zhao2019mrna, parashar2019timeloop}, as it directly determines the amount of data reuse and data movement.
Dataflows consist of three key components: loop ordering, tiling, and parallelization, which define how the dimensions are distributed across the PEs to run in parallel. %By defining a specific loop order, the dataflow inherently determines the datatype that remains {\it stationary}  between the dimensions~\cite{eyeriss}. Loop tiling and parallelization (i.e., workload partitioning) define how the dimensions are distributed across the PEs to run in parallel.

%\cite{xiao2017load,xiao2019self}  
%\HK{I added them in our bib file. However, I am not sure if we want to cite them basd on the context we have. The first work (A load balancing inspired...) is about auto-parallelization of sequential programs over an exascale system and optimization (reduce the traffic across processors, maximize core utilization in each processor, and load balancing).
%The other work is somewhat related but I found that the granularity of mapping and the focus of the paper are are quite different from those in DNN accelerator works. (e.g., in the context of DNN accelerators, data reuse is one of the key topics while the work does not consider data reuse.)}
%\TODO{HK: cite some Paul Bogdan work - A load balancing inspired optimization framework... Self-Optimizing and Self-Programming Computing Systems: A Combined Compiler, Complex Networks.... if appropriate.}
%, entails a heavier impact in the performance of the accelerator.

%Regarding this, there are certain spatial, temporal and spatio-temporal reuse opportunities that an accelerator can leverage.

%The spatial reuse entails that the same data can be used by two different PEs simultaneously, being related to multicast or broadcast support in the NoC. Temporal reuse means that the same data can stay in the same PE for some iterations while it computes different output activations using that value, and it requires buffers at PE level. Spatio-temporal reuse means that data can be forwarded between PEs so that it can be used later. 
%In this sense, every accelerator has an intrinsic dataflow, which is usually fixed. For instance, Eyeriss\cite{eyeriss} and TPU\cite{} are two good examples.
%\begin{figure}[t]
%\setlength{\abovecaptionskip}{0pt}
%\setlength{\belowcaptionskip}{-4pt}
%\centering
%\includegraphics[width=0.85\columnwidth]{fig/dimensions.pdf}
%%\vspace{-0.2cm}
%\caption{\it Convolution data operation}
%\label{fig:dataspace}
%\vspace{-0.4cm}
%\end{figure}


\betterparagraph{Communication} 
DNN accelerators involve three phases of communication~\cite{maeri} handled 
by the NoC.
(1) \textit{Distribution} is a few-to-many flow that involves sending inputs and weights to the PEs via unicasts or multicasts or broadcasts depending on the partitioning strategy of the dataflow.
(2) \textit{Local} forwarding involves data reuse within the PE array via inter-PE input/weight/partial-sum forwarding.
(3) \textit{Collection} involves writing the final outputs back to the global SRAM.

%However, when scaling-out an accelerator, another NoC level arises. In this scenario, we can talk about the on-chip level, referring as the NoC inside each cluster or chiplets, or the off-chip level, when we allude to the NoC connecting the chiplets through the on-package level.

%\betterparagraph{Scale-out} 
%Scaling out introduces 
%a second level for both the dataflow and communication.
%For the dataflow, 
%the DNN dimensions can be partitioned across chiplets (for parallelization), 
%and then further within the array.
%For communication, the first level NoC connects a global SRAM to the chiplets, followed by a second level within the chiplets.

%Therefore, scaling-out allows us to partition the dimensions between the chips, while at the same time each chiplet will condition the data movement by implying its on-chip level dataflow.

\begin{comment}
\RG{In progress}

Tackling the temporal reuse alone, several different strategies can be followed. For instance, each PE could fetch new data, that is weights and inputs, at every cycle and compute the MAC operation. Another approach could be to make each PE hold the same weight value until all the calculations involving it are done, reducing the movement of filters. Opposite to this, we can make them hold the input instead of the weights. These different approaches lead to different dataflow groups: No local reuse (NLR), Weight Stationary (WS), Input Stationary (IS) and others~\cite{eyeriss}, and in the past the accelerator systems tended to stick to one of them by exploiting its capabilities statically. This dataflow space is huge and its exploration is an actively research topic, due to the impact in performance and broadcast opportunities that it produces.
The fact that we have billions of operations but only millions of parameters show the potential reuse opportunities in a NN. As we will see later, depending on the available hardware resources, the targeted NN and layer and the dataflow choice, the performance of the accelerator can vary substantially.
%As an example, Fig. \ref{fig:chip_data_is} shows how when using an IS-like dataflow, weight broadcasting opportunities may appear, though it highly depends on the hardware resources and the dataflow implementation.


%\textcolor{red}{NoCs and interposer: }
While there are many electrical NoC topologies available to interconnect PEs and memory, state-of-the-art DNN accelerators tend to be designed using buses or trees~\cite{maeri}, and other options include meshes as well. They provide good performance and energy efficiency up to a certain level of cores, while maintaining a low area and power consumption. However, these NoCs are not as flexible and have to face performance challenges. Specifically,  when the number of PEs increases, the NoC requirements become more and more tough, and the whole system urges a way to route the data in a flexible, scalable manner.

In addition, the PEs can be grouped together to create clusters to allow heterogeneous mappings and reduce costs.
When clustering the PEs, the dataflow search becomes even more complex and non-intuitive, with different levels of parallelism, and the impact in the throughput and runtime metrics is not negligible. % (The community still lacks a tool for a dataflow space exploration)
By using clusters, another NoC level arises. In this scenario, we can talk about the on-chip level, referring as the NoC inside each cluster or chiplets, or the off-chip level, when we allude to the NoC connecting the clusters in the upper on-package level.

As for the off-chip NoC, a growing tendency for the accelerators has been to rely on  interposers \cite{Kim2019ArchitectureCA}. This technology allows 2.5D IC designs, interconnecting totally independent chiplets by using a passive interposer fabric beneath them. This way, the connections don't need to go all the way down to the die, being mapped across it and go up again, which is power consuming. Instead, the interposer allows fast communication between chiplets and only those connections leaving the SoC need to be mapped down. Moreover, each chiplet can be manufactured separately and using different technologies. Notwithstanding, its limited space availability does not allow for broadcast or high-bandwidth long-range communications. [\RG{REDUNDANT}]
\end{comment}

\subsection{2.5D Integration}
\label{sec:interposer}
\vspace{-1mm}

2.5D systems refer to the integration of multiple discrete chips (often called chiplets) within a package, either over a silicon interposer~\cite{chips_dac2019}, or via other packaging technologies. 
2.5D integration is promising 
for multiple reasons: yield (smaller chiplets have better yields than large monolithic dies), reusability (chipletization can enable plug-and-play designs, enabling reusability of the same IP across different SoCs), and cost (it is more cost-effective to integrate multiple chiplets on a package than design a complex monolithic die each time).


A silicon interposer is effectively a large chip upon which other smaller chiplet dies can be
stacked.
Thus wires on the interposer can operate at the same latency as on-chip wires.
However, the micro-bumps used to connect
the individual die to the interposer are $\sim$40$\upmu$m in state-of-the-art TSMC processes~\cite{chips_dac2019}.
While this is much finer than 
board-level integration via C4 bumps ($\sim$180$\upmu$m), it is much wider than that of NoCs, limiting the effective inter-chiplet bandwidth.
In other words, 
the effective bandwidth of a chiplet-to-chiplet connection gets limited by the number of microbumps that can fit over the surface area of the chiplet~\cite{chips_dac2019}.  

%\TK{Add to Section 2B: communication phases: distribution and collection}

%Limited interposer bandwidth
%imposes a key challenge for a scale-out DNN accelerator since 
%The communication pattern in a 
%scale-out DNN accelerator is few-to-many-to-few.
%During the distribution 
%phase 
%(\autoref{sec:dnnaccelerators}) 
%in a scale-out accelerator, 
%SRAM chiplets distribute model inputs and weights to multiple accelerator chiplets; during the collection phase, the final outputs from these chiplets
%are written back to the SRAM.
In a scale-out DNN accelerator, limited interposer bandwidth
imposes a key challenge since it determines the read and write bandwidth from the global SRAM.
While collection (i.e., write) can be hidden behind compute delay, distribution (i.e., read) is in the critical path~\cite{shao2019simba}, and enhancing its bandwidth is the focus of this work.
%\TODO{HK: cite some 2.5D-based DNN accelerators, if any.
%}
%\HK{Added one}

%\TK{Some numbers for BW}.


%\TK{introduce chipletization for scale-out and cost reduction. And talk about interposer BW challenges}

%\TK{Hyoukjun and Tushar will take a first cut}
%\TK{Add a figure or table showing electrical BW - MCM, interposer, or fancier technologies. Limited by pin bandwidth.}


%Wires are relatively cheap on-chip
%since the area of an IP block is dominated by logic, not I/O, since the
%minimum wire pitch in modern technology nodes is 0.09μm. For a
%chiplet, however, C4 bumps to connect to the interposer are much
%wider such as 180μm, and can potentially completely dominate
%the area of a chiplet, as we quantify later in Section 5.1. Moreover,
%chiplet-to-chiplet interconnections are generated through the interposer
%layer which has larger dimensions and longer wire length
%compared to monolithic 2D design, so additional I/O drivers are
%necessary for each input and output to drive the signals without
%any loss.

\insertWideFigure{Partitioning_Strategies}{Three tensor partitioning strategies across chiplets (a,b,c). Cp refers to chiplet. Based on the strategies, we construct three strategies as shown in (d). The replicated tensors are broadcast, while the partitiond tensors are unicast using the distribution network.
%\TODO{HK: typo (FP) in strategy name column - first row}
%\HK{Thank you for the catch. I fixed it.}
}

\insertWideFigure{Motivation_BW_Impact}{The impact of bandwidth on throughput. We analyze a classification network, Resnet50~\cite{resnet}, and a segmentation network, UNet~\cite{unet} varying partitioning strategies. High-res and low-res layers indicate layers with larger/smaller activation height/width compared to the number of channels. Residual, FC, and Up-Conv indicate residual links, fully-connected layer, and up-scale convolutions. \vspace{-1mm}}

\vspace{-3mm}
\subsection{Wireless In-Package Communication}
\label{sec:wnoc}
\vspace{-1mm}
%\TODO{RG: Add some details on wireless channel - no fading, static, controlled.}
Recent years have seen the emergence of a wide variety of on-chip antennas \cite{Cheema2013, Pano2019} and transceivers \cite{Yu2014, Tokgoz2018} in the mmWave-THz bands for ultra-high speed, ultra-short range wireless communications. %Their on-chip integration is possible thanks to the constant improvements of RF-CMOS technology that enabled the use of spectrum beyond 60 GHz. 
Several works have shown that, at these bands, it is possible to reach speeds of upto 100 Gb/s. Figure \ref{fig:power_dr} shows how the area and power consumption scale with the data rate, based on the analysis of 70+ short-range transceivers (see \cite{Tasolamprou2019, Yu2014, Tokgoz2018} and references therein) with different modulations and technologies, but mostly around 65nm CMOS, including the needed circuitry.

Among the applications for this technology, we highlight wireless in-package communications. In this paradigm, wireless interfaces are co-integrated with the computing elements of a multiprocessor and use the system package as the wireless propagation medium. This in-package channel will be static and controlled. %Several works \cite{Tasolamprou2019, Timoneda2018ADAPT} have shown that the package dimensions and materials determine the characteristics of the channel, and that these are compatible with low-power, ultra-reliable broadband communication. 
As an example, the attenuation below 30 dBs with a loss exponent of 1.32 achieved in \cite{Timoneda2018ADAPT} is compatible with the 65-nm transceiver from \cite{Yu2014}, which operates at upto 48 Gb/s with a Bit Error Rate (BER) below 10\textsuperscript{-12}, taking 0.8 mm\textsuperscript{2} and consuming 2 pJ/bit. At newer technologies and further optimizing the circuit topology, even better figures may be achieved.

%enhancing communication among cores regardless of their location. Therefore, 
%. Such wireless
%The definition of wireless in-package communication applies to both planar \cite{replica} and 2.5D architectures \cite{ahmed2018asymmetric}. %At the chip level, wireless communications have been explored from the transceiver \cite{Yu2014} up to the architecture \cite{replica}. %At the package level, wireless communications are relatively less explored even though efforts exist in antenna design \cite{Pano2019}, channel characterization \cite{Narde2019} and network design \cite{ahmed2018asymmetric}. 

%The aim is to alleviate the communication bottleneck of current architectures with the inherent broadcast capabilities and low latency of this technology.

By not needing to lay down wires between transmitter and receiver, wireless technology offers additional benefits at the package level, such as inherent broadcast capabilities and low latency. In particular, it increases the available bandwidth and reduces cost as it does not depend on pin limitations and wire routing constraints. It also allows to dynamically change the topology as each receiver can decide at run-time whether to process information being transmitted. For instance, one option to do so is by broadcasting the scheduling information to all receivers beforehand. Finally, broadcast is scalable in the sense that additional chiplets only need to incorporate a transceiver, and not extra off-chip wiring, to participate in the communication. While provisioning wires to enable broadcast can be prohibitive, and even then multiple hops are unavoidable, wireless bypasses those problems.


%As illustrated next, these properties are very desirable in the domain of machine learning accelerators.





% \textbf{Flexibility.} An important advantage of wireless links is the flexibility they can provide. When a transmitter is sending data through the package, each receiver can decide at run-time whether to process/acquire the information or not. This means that this technology allows to virtually map different typologies at every cycle, which enables dataflow adaptability at cycle level.

% For instance some of the configurations could facilitate multicasts, and some others unicasts. On the contrary, wired topologies are fixed and very few of them seek to achieve flexible data movements. 
% Within this flexibility, WNoCs inherently allow broadcast transmissions due to their nature. The data is modulated at the transmitter and sent through the antenna, which will allow the propagation of the information across the package through EM waves to reach all the receiver antennas within range. This broadcast feature is particularly desirable in an accelerator NoC, since many dataflows try to spatially reuse the data across different PEs.



% \textbf{Bandwidth.}
% While in the on-chip communications the bandwidth is not usually a problem, on-package links suffer from bandwidth bottlenecks. In wired off-chip communications, the chiplets to be interconnected have limited space for pins, which limits the bandwidth due to large bumps pitch. Therefore, off-chip links are costly and often assume neighbor-to-neighbor or other point-to-point communications, mainly because other than those are prohibitive. Consequently, they are limited to short range communications, which in turn made most of the design approaches to develop towards that restricted scheme. A common design approach is to place an active NoC on the interposer to interconnect the off-chip chiplets. In this case, the NoC routes the traffic through thin links to the chiplets which turns in limited bandwidth, besides being a bottleneck for scalability and broadcast.
% However, WNoCs enable long range communications within package and can provide higher bandwidth than interposer-based NoCs, even between detached chips, while supporting multicasting natively and at low latency.




% \textbf{Scalability.} When NoCs try to scale, most of them face multi-hop problems, enlarged areas and power consumption or even layout difficulties. On the contrary, WNoCs escalate linearly when the number of cores in the network grows. In other words, increasing the number of receivers does not exponentially increase the whole NoC as in a tree or a mesh, but the only overheads are the receivers themselves. 
% For instance, in a tree-based NoC, when the number of leaves increases, it entails a change in the whole network to feed all the cores. This means more switches and metal interconnects through all the NoC. In a bus, larger distances increase the complexity and consumption exponentially. Nevertheless, in a WNoC adding cores is as simple as adding a receiver with them, since they will be able to receive the data no matter where it is located in the package. On the contrary, long-range direct-wired interconnections are becoming challenging for traditional NoCs and in some cases they are just not feasible to lay out.











%\label{broadcast}

%\textbf{Broadcast.} Wireless Networks-on-Chip inherently allow broadcast transmissions due to their nature. The data is modulated at the transmitter and sent through the antenna, which will allow the propagation of the information across the package through EM waves to reach all the receiver antennas within range. The receivers can then choose whether to acquire the signal or not. In this case, the network does not have to spend resources such as multiple switches in replicating the data to reach every PE.
%This broadcast feature is particularly desirable in an accelerator NoC, since many dataflows try to spatially reuse the data across different PEs.
%In fact, for a WNoC, the more broadcast traffic is needed, the better it will perform.

%\label{latency}
%\textbf{Latency.} Due to the wireless propagation, the waves carrying the information travel around the package at a speed close to that of light. This ensures an almost distance independent communication, granting a reduced latency level. In addition, this topology does not require routing or multi-hop links from the sender to the receiver, saving time and intermediary circuitry.
%This not only helps reducing the overall latency, but also facilitates the layout task because now the PEs allocation is not so critical and thus leaves more room to place wired components whose position can critically affect the performance. (this is not so important in an accelerator?)

%\label{Flexibility}

%\textbf{Flexibility.} Another key advantage of wireless links is the flexibility they can provide. As already mentioned, when a transmitter is sending data through the package, each receiver can decide at run-time whether to process the information or not. 
%This means that this technology allows to virtually map different typologies at every cycle. For instance some of them could facilitate multicasts, and some others unicasts. On the contrary, wired topologies are fixed and very few of them seek to achieve flexible data movements. 

%[Additionally, since the transmitted data will have to be serialized, the WNoC can also offer precision adaptability between layers as well as error flexibility by changing the wireless BER, allowing the whole system to save power when less accuracy is required. As studied in [Bit-Serial paper], per layer precision can provide lossless accuracy and energy savings.] [remove?]

%Moreover, other well known techniques at large scale wireless links could be applied. For instance, even though the usually chosen on-chip communication schemes are simple such as OOK, complex modulations can also be used to improve the spectrum efficiency. In terms of multiple access to the shared medium, multiple frequency channels have been proposed in [Yu]. Beamforming, which allows spatial multiplexing, has been  studied in []. CDMA techniques are also possible. 
%The drawback for all these large-scale options is the increased complexity of the transceivers, which affects the area and power consumptions.
%(not sure about including this)

%(Mention technology maturity gap --> + spectrum efficiency expected.)




%This appealing features, however, come at an area and power overhead and limited datarates.

%\begin{figure*}[h]
%\setlength{\abovecaptionskip}{0pt}
%\setlength{\belowcaptionskip}{-4pt}
%\centering
%\includegraphics[width=2\columnwidth]{./fig/thr_junt.pdf}
%\includegraphics[width=2\columnwidth]{./fig/thr_junt.pdf}
%\vspace{-0.2cm}
%\caption{\it Dataflow performance comparison}
%\label{fig:dataflows}
%\vspace{-0.4cm}
%\end{figure*} 

==> backup/05-evaluations.tex <==
\section{Evaluation}
\label{sec:evaluations}
%\vspace{-2mm}

%\HK{Latency (runtime) and Energy varying BW, chiplet size for each layer type. Do we have extra parameters to explore in WNoC?}

\subsection{Methodology}
\label{sec:methodology}
We list up hardware parameters, workloads, partitioning strategy, and NoP characteristics in~\autoref{table:eval_setting}.
%
To compute the throughput, we use an open source DNN accelerator cost model, MAESTRO~\cite{maestro}, which is validated with average accuracy of 96.1\% against RTL simulation and measurements.
% adopted in XX YY.. (HK: I think this might be too much so I am not including this at this point)
%
MAESTRO takes into consideration the latency, bandwidth, and multicasting characteristics of the different NoPs.

%Considering the characteristics of interposer and wireless network, we apply appropriate interconnect parameters as shown in~\autoref{table:eval_setting}.


%Explain the simulator used: explain how does it models area/power bus, and latency... new changes from publication..
%Analytic model, not cycle-accurate.
%Explain DNN model used
%Explain on-chip vs off-chip models for the comparisons in WnoC vs wired. 
%\textcolor{red}{TRXs models:}

%In order to compute energy consumption of wireless transmissions, we have that \begin{equation}
%\begin{gathered}
%\label{equation:wireless_energy}
%E_{broadcast} = E_{tx} + N_cE_{rx}\\
%E_{unicast} = E_{tx} + E_{rx},
%\end{gathered}
%\end{equation}
%where $E_{tx} = P_{tx}/R$, $E_{rx} = P_{rx}/R$ represent energy consumption of the transmitter and receiver, given by their respective power consumption figures $P_{tx}$ and $P_{rx}$ and the transmission data rate $R$. 
On the one hand, the energy of a wired NoP is obtained by computing the average number of hops multiplied by the per-hop energy. On the other hand, to estimate the area and power of the wireless NoP, we select conservative and aggressive design points from~\autoref{fig:area_dr} at the required transmission rates. Note that~\autoref{fig:area_dr} assumes a single transmitter and receiver with a 60\%/40\% ratio. This allows to model the energy of both unicasts, where only the required receiver is active while others remain powered off to save energy; and broadcasts (multicasts), where the transmitter at the SRAM and all receivers (a set of receivers) are active. 
%to achieve a single-hop single-cycle transmission. This can be applied to multicasts as well, implying that the transmitter and only the required receivers consume power.

%In fact, every hop will add its link energy to the total energy consumption for that transmission, which grows fast especially in broadcast situations. %In this scenarios, the total number of hops grows up to $k^2-1$ in a $k \times k$ mesh NoC.

%\TODO{RG: comment on how energy can be obtained from power and datarate, and relate to Fig.2. Add energy-related comments from OrthoNoC paper}
\begin{comment}


State-of-the-art wireless TRXs have been studied in Fig. \ref{fig:area_dr} and \ref{fig:power_dr} to benchmark the actual datarate and consumption.

Both optimistic and pessimistic approaches have been computed. For the pessimistic approach, only on-chip TRXs implementations have been included, whereas for the optimistic fit both on-chip and long range TRXs have been used. In the optimistic case, the paretto optimal frontier has been obtained in order to work with the best TRXs published at every datarate.

In the power fitting, a normalization factor has been applied since it would not be fair to compare TRXs designed for different ranges or different bit error ratio (BER), as the amplifier consumption of the transmitter and receiver varies.
Moreover, a maturity factor has been appied as a weight for the fitting, which gives more relevance to the TRXs that provide better datarate in relation to its carrier frequency. In a sense, these TRXs are more developed and have better spectral efficiency.


In a general manycore wireless system, where all the cores both transmit and receive data, the power and area allocation of the total TRX into the transmitter and receiver is not so relevant. However, in a wireless distribution network, we will have few transmitters and several receivers.
\HK{This seems more like results..}
After studying the different TRX implementations, an average of 50.6\% of the area , and a 46.6\% of the power were consumed in the receiver and the rest in the transmitter. However, this is an implementation choice, because the complexity of the TRXs can be given over the transmitter or the receiver as desired. For instance, the transmitter amplifier can have more gain at the expense of a reduced consumption in the receiver to maintain a safe link budget. As an optimistic reference, we took 35\% for both power and area consumption load in the wireless receiver.

To compare the datarate of Wireless Networks on Chip TRXs with the electrical bandwidth, defined as the unique number of bytes transmitted in a cycle, we assume a clock frequency of 200 MHz as a baseline (cite Eyeriss?)

As for the NoC bandwidth of state-of-the-art accelerators, unrestricted bandwidth has been assumed on-chip, and 8 Bytes/cycle has been assumed off-chip.  
%Detailed explanation of the models and how they've been collected.
%TRXs area-power/throughput-BW

%To obtain the available bandwidth at off-chip level by assuming 256 PEs per chiplet, being conservative. Then, the size of the chiplet limits the room for bumps both at the chip and the interposer.



%Moreover, the WNoC will work whether the interposer is there or not, so we can choose to include it to make a cross-technology design, as recent trends suggest.%, or not, if we dont need wires..)

\end{comment}

\subsection{Results}
\label{sec:results}
%\TODO{Add energy results, comparing wireless and wired approaches. Maybe this could be done extracting from the dataflows the num. unicasts and num. broadcasts for each model, and then convert it to comms energy, and finally give a Joule/MAC metric. Having this numbers also helps justify the effort to improve broadcast/multicast energy \\@HK, how easy is it to extract those numbers from dataflow descriptions or MAESTRO output? Can we have some statistics on unicasts/broadcasts? and relate it with wired comms energy, maybe taking Table I and considering the num. hops? \\RG/SA: Put those stats into wireless comms energy numbers - maybe as extra subsection.}
%\HK{Energy numbers are in}

%\insertWideFigure{EvalResults_Integrated}{(a),(b) Throughput analysis of conservative(C)/aggressive(A) designs of interposer- and WIENNA-based 2.5D accelerators. (c),(d) The impact of cluster sizes under three partitioning strategies. \vspace{-2mm}}


%\insertWideFigure{Eval_MultcastFactor}{Average multicast factor (number of received data across all the chiplets / number of sent data from global SRAM) for each layer types in the evaluated DNN models, (a) Resnet50 and (b) UNet. In this analysis, we apply the cluster size of 64, which results in 256 chiplets.}

We compare the performance of interposer-based and WIENNA accelerators in~\autoref{fig:EvalResults} and their energy in~\autoref{fig:Eval_Energy}. Also, we investigate the impact of chiplet size in~\autoref{fig:ClusterSz}.


\betterparagraph{Throughput Improvements}
As presented in~\autoref{fig:EvalResults}, WIENNA improves the end-to-end throughput by 2.7-5.1$\times$ on Resnet50 and 2.2-3.8$\times$ on UNet.
%
%Although WIENNA significantly improves the end-to-end throughput, 
Performance can be improved further if we realize that the partitioning strategy may fundamentally limit the performance on specific layers.
%
For example, on high-resolution layers in Resnet50, KP-CP and NP-CP partitioning strategy limits the performance so both of interposer and WIENNA provides similar throuhgput.
%
However, in rest of layers, WIENNA successfully exploits the potential of each partitioning strategy.
%
In the end-to-end charts of~\autoref{fig:EvalResults}, we present results based on adaptive partitioning strategy where we select the most efficient strategy for each layer.
%
The adaptive partitioning strategy improved the throughput further by 4.7\% and 9.1\% on average on Resnet50 and UNet, respectively, compared to the best partitioning strategy (KP-CP) across all layers.


\input{Tables/EvalSettingTable.tex}


\insertWideFigure{EvalResults}{Throughput analysis of conservative (C) and aggressive (A) designs of interposer- and WIENNA-based 2.5D accelerators.}

\insertWideFigure{Eval_Energy}{Data distribution energy for input activations and filters 
% from global SRAM to chiplets 
in interposer- and WIENNA-based 2.5D accelerators. Inset  
%We show energy consumption for each input tensor (input activation and filter). 
(c) summarizes the end-to-end energy reduction by WIENNA compared to the interposer-based 2.5D accelerator.}

\insertWideFigure{Eval_MultcastFactor}{Average multicast factor (number of received data across all the chiplets / number of sent data from global SRAM) for each layer types in the evaluated DNN models, (a) Resnet50 and (b) UNet. In this analysis, we apply the cluster size of 64, which results in 256 chiplets.}

\insertWideFigure{ClusterSz}{The impact of cluster sizes under three partitioning strategies. (a) presents results on Resnet50, and (b) presents results on UNet}



\betterparagraph{Impact of Wireless Broadcast}
Although aggressive interposer (interposer A) and conservative WIENNA (WIENNA C) have the same bandwidth as listed in~\autoref{table:eval_setting}, their performance dramatically differs.
%
WIENNA C provides 2.58$\times$ and 2.21$\times$ higher throughput than interposer A.
%
The difference is based on the single-cycle broadcasting of the wireless NoP, much faster than the multi-hop wired baseline.
%The difference is based on the benefits of wireless interconnect that enables single cycle broadcasting, as opposed to the multi-hop latency in the baseline.
%
The feature is critical in DNN traffic since many partition methods require heavy broadcasting as we observed in~\autoref{fig:Partitioning_Strategies}.
%

The wireless broadcast also affects the energy consumption. %for communication.
%
~\autoref{fig:Eval_Energy} compares the energy consumed in the distribution (from SRAM to chiplets) of input activations and filters in WIENNA and the baseline. \hl{WIENNA A or C? Interposer A or C?}
%
Across all the partitioning strategies and layers, WIENNA leads to an average energy reduction of 38.2\%.
%
The energy saving is based on both the efficient multicast support via wireless NoP and the ample multicast opportunities from each partitioning strategy.

\hl{See commented text in evaluation.tex. This text shall be eliminated or repurposed now that the multicast factor figure has been eliminated. We may want to just give the numbers, without the figure. Also, we can think on removing Figure 5.}


%
%To show the quantified multicast opportunities, ~\autoref{fig:Eval_MultcastFactor} plots the multicast factor, which 
%The multicast factor is the average number of receiver chiplets when the global SRAM sends data (i.e., number of received data by all chiplets / number of sent data from the global SRAM), and its maximum corresponds to the number of chiplets, which indicates broadcasting.
%

%Each partitioning strategy exploits different amount of spatial reuse (i.e., multicast) from different input tensors (input activation or filter).
%
%The layer type determines the multicast factor within each partitioning strategy.
%
%When the multicast factor is high, the energy reduction was also high.
%
%For example, KP-CP partitioning strategy has the highest overall multicast factor among three partitioning strategies, which led to the highest energy reduction, as shown in~\autoref{fig:Eval_Energy}(c).
%


\betterparagraph{Impact of the Number of Chiplets} Assuming a total of 16384K PEs,~\autoref{fig:ClusterSz} shows the impact of increasing the number PEs in each chiplet and, thus, integrating fewer but larger chiplets. %(i.e., chiplet size), which can be translated into the number of Chiplets as we fix the total number of PEs (e.g., 64 PEs/Chiplet can be translated into 16384 / 64 = 256 Chiplets).
%
For the interposer NoP, we adapt the number of hops to the resulting number of chiplets.
%
%We apply KP-CP partitioning strategy that can utilize more number of chiplets because output channel dimension (K) is large in many layers and we vary the number of chiplets in this analysis from 32 to 256.

Since the total number of PEs is fixed, less chiplets lead to more traffic per chiplet. %as more data needs to be fed for each computing tile mapped on each chiplet.
%
However, more elements also can be broadcasted in such cases.
%
Also, the utilization of chiplets and PEs in each chiplet depends on layer type and the partitioning strategy, which is another major factor determines overall throughput.
%
As a consequence, we do not observe monotonic change of the throughput for all the cases.
%
Overall, we observe WIENNA is more affected by the cluster sizes compared to interposer.
%
As we change the number of PEs in each chiplet from 64 to 512, the throughput of interposer and WIENNA vary 62.5\% and 77.5\%, on average, across both models.
%
However, this also implies that WIENNA contains more potential for improvements via further optimization of other design parameters like number of chiplets.




\begin{comment}

\begin{figure}[h]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-4pt}
\centering
\includegraphics[width=0.8\columnwidth]{fig/RUNTIME_bar_stacked.pdf}
%\vspace{-0.2cm}
\caption{\it Runtime analysis - remove}
\label{fig:runtime_bars}
\vspace{-0.4cm}
\end{figure}
%Numbers of the results
%Specific design evaluated at different dataflows..
%evaluate my design with the 2 dataflows and optimal adaptive
%Overall, we found WIENNA to be XXX times faster than ...


\begin{figure}[h]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-4pt}
\centering
\includegraphics[width=0.8\columnwidth]{fig/UNet_runtime.PNG}
%\vspace{-0.2cm}
\caption{\it draft - UNet Runtime}
\label{fig:runtime_bars}
\vspace{-0.4cm}
\end{figure}

\begin{figure}[h]
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-4pt}
\centering
\includegraphics[width=0.8\columnwidth]{fig/ResNet_runtime.PNG}
%\vspace{-0.2cm}
\caption{\it draft - ResNet Runtime}
\label{fig:runtime_bars}
\vspace{-0.4cm}
\end{figure}

\end{comment}

%\TODO{@TK: do we want to show an energy breakdown? inter/intra-chiplet wired comms, wireless comms, comuputing, etc. \\@HK: Can we obtain those from Maestro, at least the wired ones and computing?}
%\HK{We will get a plot}
